Convergence of the Chambolle-Pock Algorithm in the Absence of Monotonicity

The Chambolle-Pock algorithm (CPA), also known as the primal-dual hybrid gradient method, has gained popularity over the last decade due to its success in solving large-scale convex structured problems. This work extends its convergence analysis for problems with varying degrees of (non)monotonicity, quantified through a so-called oblique weak Minty condition on the associated primal-dual operator. Our results reveal novel stepsize and relaxation parameter ranges which do not only depend on the norm of the linear mapping, but also on its other singular values. In particular, in nonmonotone settings, in addition to the classical stepsize conditions, extra bounds on the stepsizes and relaxation parameters are required. On the other hand, in the strongly monotone setting, the relaxation parameter is allowed to exceed the classical upper bound of two. Moreover, we build upon the recently introduced class of semimonotone operators, providing sufficient convergence conditions for CPA when the individual operators are semimonotone. Since this class of operators encompasses traditional operator classes including (hypo)- and co(hypo)-monotone operators, this analysis recovers and extends existing results for CPA. Tightness of the proposed stepsize ranges is demonstrated through several examples.

==> TeX/Text/Preliminaries.tex <==
%!TEX root = ../../CP-Minty.tex

\begin{proposition}[{{\cite[Prop. 20.44]{bauschke2017Convex}}}]
  Let \(X\subseteq \R^n\) be a closed linear subspace, and \(T:\R^n\rightrightarrows\R^n\) be a set-valued operator.
  % Let \(X\subseteq \R^n\) be a closed linear subspace, and let \(L_X\) be the Spingarn operator.
  Then, the following hold:
  \begin{enumerate}
    \item\label{it:spingarn:inverse} \(T^X = (T^{X^\bot})^{-1} = (T^{-1})^{X^\bot}\).
    \item\label{it:spingarn:gph} \(L_X^{-1} = L_X\) and \(\graph T = L_X(\graph(T^X))\).
    \item\label{it:spingarn:inner} Let \(x_1, u_1, x_2, u_2 \in \R^n\) and set \((y_1, v_1) = L_X(x_1, u_1)\) and \((y_2, v_2) = L_X(x_2, u_2)\). Then, \(\langle y_1 - y_2, v_1 - v_2 \rangle = \langle x_1 - x_2, u_1 - u_2 \rangle\).
    \item\label{it:spingarn:zero} \(z \in \zer T^X \Leftrightarrow (\proj_X(z), \proj_{X^\bot}(z)) \in \graph(T)\).
    % \item\label{it:spingarn:semimonotone} If \(T\) is \((\sigma, \rho)\)\hyp{}semimonotone, then \(T^X\) is \((\nu, \nu)\)\hyp{}semimonotone with \(\nu = \min\{\sigma,\rho\}\).
    % \item\label{it:spingarn:maxsemimonotone} If \(T\) is maximally \((\sigma, \rho)\)\hyp{}semimonotone, then \(T^X\) is maximally \((\nu, \nu)\)\hyp{}semimonotone with \(\nu = \min\{\sigma,\rho\}\).
  \end{enumerate}

  % \begin{proof}
  %   \begin{proofitemize}
  %     \item \ref{it:spingarn:inverse}-\ref{it:spingarn:zero} See \cite[Prop. 20.44]{bauschke2017Convex}.
  %     \item \ref{it:spingarn:semimonotone} Let \((x_1, u_1), (x_2, u_2) \in \graph(T)\) and set \((y_1, v_1) = L_X(x_1, u_1)\) and \((y_2, v_2) = L_X(x_2, u_2)\).
  %     By orthogonality, it holds that
  %     \begin{align*}
  %       \nrm{y_1 - y_2}^2 &= \nrm{\proj_X(x_1-x_2)}^2 + \nrm{\proj_{X^\bot}(u_1-u_2)}^2\\
  %       \nrm{v_1 - v_2}^2 &= \nrm{\proj_X(u_1-u_2)}^2 + \nrm{\proj_{X^\bot}(x_1-x_2)}^2.
  %     \end{align*} 
  %     Then, by \ref{it:spingarn:inner} and \Cref{def:semimonotonicity},
  %     \begin{align*}
  %       \inner{y_1 - y_2, v_1 - v_2} {}\geq{}& \sigma \nrm{x_1 - x_2}^2 + \rho \nrm{u_1 - u_2}^2\\
  %       {}={}& \sigma \nrm{\proj_X(x_1 - x_2)}^2 + \rho \nrm{\proj_{X^\bot}(u_1-u_2)}^2\\
  %       & + \sigma \nrm{\proj_{X^\bot}(x_1-x_2)}^2 + \rho \nrm{\proj_X(u_1-u_2)}^2\\
  %       {}\geq{}& \nu \nrm{y_1 - y_2}^2 + \nu \nrm{u_1 - u_2}^2.
  %     \end{align*} 
  %     \item \ref{it:spingarn:maxsemimonotone} Follows from \ref{it:spingarn:semimonotone} and \eqref{eq:def:partial}.
  %   \end{proofitemize}
  % \end{proof}
\end{proposition}

==> TeX/Text/Proofs/SemiMonCor.tex <==
%!TEX root = ../../../CP-Minty.tex

% \begin{appendixproof}{cor:semimon:fulldom}    
%     % First, we claim that a stepsize $\gamma>0$ such that \eqref{eq:semimon:fulldom:gamma} holds may only exist if $1+\gamma\nu > 0$. 
%     % % The ranges in \Cref{tab:semimon:domain} are obtained by noting that a $\gamma>0$ such that \eqref{eq:semimon:fulldom:gamma} holds may only exist if $1+\gamma\nu > 0$. 
%     % This will be proven by contradiction: assume a $\gamma>0$ exists satisfying \eqref{eq:semimon:fulldom:gamma} for which $1+\gamma\nu < 0$.
%     % Then, multiplying condition \eqref{eq:semimon:fulldom:gamma} by $1+\gamma\nu$, it follows that
%     % $
%     %     % &= \gamma(1 + \nu\xi) + \xi
%     %     \gamma + (1+\gamma\nu)\xi < 0.
%     % $
%     % Filling in the definition of $\nu$ and $\xi$, 
%     % % the left-hand side of \eqref{eq:proof:cor:semimon:fulldom:assertion2}
%     % this condition
%     % is equivalent to
%     % % \begin{align*}
%     % %     \gamma + (1+\gamma\nu)\xi = 
%     % %     \begin{cases}
%     % %         \gamma, &\quad \text{if } \com = 0,\\
%     % %         \gamma + (1+\gamma\tfrac{1-\theta}{2\com})\tfrac{\com}{\theta}
%     % %         = \gamma\tfrac{1+\theta}{2\theta} + \tfrac{\com}{\theta}
%     % %         , &\quad \text{otherwise}.
%     % %     \end{cases}
%     % % \end{align*}
%     % \begin{align} 
%     %     \begin{cases}
%     %         \gamma < 0, &\quad \text{if } \com = 0,\\
%     %         \gamma\tfrac{1+\theta}{2\theta} + \tfrac{\com}{\theta} < 0
%     %         , &\quad \text{otherwise},
%     %     \end{cases}
%     %     \label{eq:proof:cor:semimon:fulldom:assertion}
%     % \end{align}
%     % where $\theta \dfn \sqrt{1-4\com\mon}$. We distinguish between both cases for $\com$.
%     % \begin{proofitemize}
%     %     \item If $\com = 0$, \eqref{eq:proof:cor:semimon:fulldom:assertion} directly contradicts the assumption that the stepsize $\gamma$ is positive.
%     %     \item Otherwise, \eqref{eq:proof:cor:semimon:fulldom:assertion} implies that 
%     %     $\gamma < \tfrac{-2\com}{1+\theta}$. However, since $1 + \gamma \nu < 0$ and $\gamma > 0$, it must hold that $\nu < 0$ and
%     %     \begin{align}
%     %         \gamma > -\tfrac{1}{\nu} = \tfrac{-2\com}{1-\theta}.
%     %         \label{eq:proof:cor:semimon:fulldom:assertion:base}
%     %     \end{align}
%     %     Note that by definition, $\sign(\nu) = \sign(\mon)$. As a result, using the definition of $\theta$, the assumption $\com\mon < \tfrac{1}{4}$ and the fact that $\mon < 0$ it can be verified that $\tfrac{-2\com}{1+\theta} < \tfrac{-2\com}{1-\theta}$. Hence, no $\gamma$ may exists satisfying both \eqref{eq:proof:cor:semimon:fulldom:assertion} and \eqref{eq:proof:cor:semimon:fulldom:assertion:base}.
%     % \end{proofitemize}
%     % As in both cases a contradiction is reached, the claim is established.
%     % % $$
%     % %     \nu\xi =
%     % %     \begin{cases}
%     % %         0, &\quad \text{if } \com = 0,\\
%     % %         \tfrac{1-\sqrt{1-4\com\mon}{\sqrt{1-4\com\mon}}}
%     % %     \end{cases} \in (-\tfrac{1}{2}, +\infty)
%     % % $$
%     % % where we used that $\nu < -\tfrac{1}{\gamma}$

%     % Now, we will proof that the stepsize ranges in \Cref{tab:semimon:domain} are equivalent to the ranges implies by \eqref{eq:semimon:fulldom:gamma}. Using previous claim, we know that a stepsize $\gamma>0$ such that \eqref{eq:semimon:fulldom:gamma} holds may only exist if $1+\gamma\nu > 0$. Since we previously established that  $\sign(\nu) = \sign(\mon)$,
%     % it directly follows that this condition is always satisfied when $\mon \geq 0$, and otherwise only when
%     % $$
%     %     \gamma < -\tfrac{1}{\nu} =
%     %     \begin{cases}
%     %         -\tfrac{1}{\mon}, & \text{if }\com = 0,\\
%     %         \tfrac{-2\com}{1-\theta}, \quad \quad & \text{otherwise}.
%     %     \end{cases}
%     %     % \begin{equation}\label{eq:XiBeta}
%     %     %     \xi 
%     %     %         {}={}
%     %     %     \tfrac{\com}{\sqrt{1-4\com\mon}},  
%     %     %     \qquad% 
%     %     %     \nu 
%     %     %         {}={}
%     %     %     \begin{cases}
%     %     %         \mon, & \text{if }\com = 0,\\
%     %     %         \tfrac{1-\sqrt{1-4\com\mon}}{2\com}, \quad \quad & \text{otherwise}.
%     %     %     \end{cases}
%     %     % \end{equation}
%     % $$
%     % Subsequently, assuming $1+\gamma\nu > 0$, \eqref{eq:semimon:fulldom:gamma} holds when $\gamma + (1+\gamma\nu)\xi > 0$, which is always satisfied when $\com \geq 0$, i.e., when $\xi \geq 0$, and otherwise only when
%     % $$
%     %     \gamma > -\tfrac{\xi}{1+\nu\xi} = \tfrac{-2\com}{1+\theta}.
%     % $$
%     % As the previous conditions match the stepsize ranges provided in \Cref{tab:semimon:domain}, the first part of the proof is completed.

%     \begin{proofitemize}
%         \item \ref{cor:semimon:Lip}: 
%           Take $(u,v), (\other{u}, \other{v}) \in \gph J_{\gamma A}$. By semimonotonicity of \(A\) at \(v\), \(\other{v}\), and using the fact that  
%     \(
%         \tfrac1{\gamma}(u-v) \in Av,
%     \) 
%     \(
%         \tfrac1{\gamma}(\other{u}-\other{v}) \in A\other{v}
%     \), we have 
%     \begin{align*}
%         \mon \nrm{v-\other{v}}^2 + \com \gamma^{-2} \nrm{(u-v)-(\other{u}-\other{v})}^2 &\leq \gamma^{-1}\inner{(u-v)-(\other{u}-\other{v}), v-\other{v}}.
%         % \\
%         % & = \gamma^{-1}\inner{u-v, x-y} - \gamma^{-1}\nrm{x-y}.
%     \end{align*}
%     Expanding the last term in the left-hand side and rearranging, we get
%     \begin{equation}\label{eq:cor:semimon:inequality}
%         \begin{aligned}
%             \left(1 + \mon\gamma + \com \gamma^{-1}\right)\nrm{v-\other{v}}^2 + \com \gamma^{-1}\nrm{u-\other{u}}^2 &\leq \left(1 + 2 \com \gamma^{-1}\right)\inner{u-\other{u},v-\other{v}}\\
%             & \leq \left|1 + 2 \com \gamma^{-1}\right|\nrm{u-\other{u}}\nrm{v-\other{v}}.
%         \end{aligned}
%     \end{equation}
%     By \Cref{it:lem:quadratic:solutions} it follows that \Cref{tab:semimon:domain} provides all strictly positive solutions $\gamma$ of \(1 + \mon\gamma + \com \gamma^{-1} > 0\). Hence, if \(u=\other{u}\) then necessarily \(v=\other{v}\) and the Lipschitz inequality holds trivially. Otherwise, divide both sides by \(\|u-\other{u}\|^2\) to obtain 
%     \begin{equation*}
%             \left(1 + \mon\gamma + \com \gamma^{-1}\right)\omega^2 - \left|1 + 2 \com \gamma^{-1}\right| \omega + \com \gamma^{-1} \leq 0.
%     \end{equation*}
%     where     
%     \(
%         \omega \dfn \tfrac{\nrm{x-y}}{\nrm{u-v}}    
%     \). 
%     Solving this quadratic inequality for $\omega$, yields the claimed Lipschitz modulus. 

%     \item \ref{cor:semimon:resolvent}:
%     \begin{proofitemize}
%         \item
%         Consider the case \([\mon]_+[\com]_+ = \tfrac14\). According to  \cref{tab:semimon:domain}, it holds that $\gamma \in (0, +\infty)$. 
%         First, suppose that $J_{\gamma A}$ has full domain, \ie \(\range{\id + \gamma A} = \R^n\). Fix \(v\in \R^n\). Then, there exists \((x,y)\in \graph A\) such that \(v = x + \gamma y\). By  \Cref{it:prop:semi:young:3}, \(y = 2\mu x + c\) for some \(c\in \R\)  and some \(x\in \dom A\), and therefore, \(v = (1+ 2\gamma \mu) x +c \gamma\). Since \(1+ 2\gamma \mu>0\) and the choice of \(v\) was arbitrary, necessarily \(\dom A = \R^n\), and as such \(A\) is maximally \((\mu,\rho)\)-semimonotone, see \Cref{it:prop:semi:young:3:maximal}. 

%         Now suppose that $A$ is maximally $(\mon, \com)$\hyp{}semimonotone then 
%         by definition it is maximally monotone and therefore by Minty's theorem \cite[Thm. 21.1]{bauschke2017Convex} the resolvent $J_{\gamma A}$ has full domain.  

%         % First, consider the case where \([\mon]_+[\com]_+ = \tfrac14\).
%         % Then, $\gamma \in (0, +\infty)$ and by \Cref{it:prop:semi:young:3} it follows that there exists a $c \in \R^n$ such that
%         % \[\gph A = \set{(x, y) \in \pazocal{X} \times \pazocal{Y}}[y = 2 \mu x + c]\] for some $\pazocal{X} \subseteq \R^n$ and $\pazocal{Y} \subseteq \R^n$.

%         % $\Rightarrow$ If $J_{\gamma A}$ has full domain, then by definition \(\range{\id + \gamma A} = \R^n\). Since 
%         % \[\gph(\id + \gamma A) = \set{(x, y) \in \pazocal{X} \times \pazocal{Y}}[y = (1 + 2 \gamma \mu) x + \gamma c]\]
%         % and $1 + 2 \gamma \mu > 0$, this may only hold when $\pazocal{X} = \pazocal{Y} = \R^n$, i.e., when $A = T$. Therefore, $A$ is maximally $(\mon, \com)$\hyp{}semimonotone owing to \Cref{it:prop:semi:young:3:maximal}.

%         % $\Leftarrow$ If $A$ is maximally $(\mon, \com)$\hyp{}semimonotone then 
%         % by definition it is maximally monotone and therefore by Minty's theorem \cite[Thm. 21.1]{bauschke2017Convex}
%         % % the operator $\id + \gamma A$ has full range, i.e.,
%         % the resolvent $J_{\gamma A}$ has full domain.  
%         \item
%         Now, consider the case where $\mon\com < \tfrac14$. Define $\theta \dfn \sqrt{1-4\com\mon}$ and let \(\nu \dfn \tfrac{2\mon}{1+\theta}\), \(\xi \dfn \tfrac{\com}{\theta}\) and 
%         \(\omega \dfn \tfrac{\gamma}{1+\gamma\nu}\).
%         % First, consider the following inequalities:
%         % \begin{itemize}
%         %     \item \(1+\gamma\nu > 0\): By definition of \(\nu\) and positivity of \(\gamma\), this inequality holds
%         %     When \(\mon \geq 0\), then \(\nu \geq 0\) and thus \(1+\gamma\nu > 0\) always holds. Otherwise, it holds if and only if
%         %     \[
%         %         \gamma < -\tfrac{1}{\nu} = -\tfrac{1+\theta}{2\mon}
%         %     \]
%         %     which is implied by \Cref{tab:semimon:domain}.
%         %     \item \(\omega + \xi > 0\):
%         % \end{itemize}
%         When $\gamma$ is selected according to \Cref{tab:semimon:domain}, it holds that \(1+\gamma\nu > 0\) (since $\gamma < -\tfrac{1}{\nu} = -\tfrac{1+\theta}{2\mon}$ when \(\nu < 0\)) so that \(\omega + \xi > 0\) holds, since
%         \begin{align*}
%             \tfrac{\gamma}{1+\gamma\nu} + \tfrac{\com}{\theta} > 0
%                 {}\stackrel{1+\gamma\nu \,>\, 0}{\Longleftrightarrow}{}
%             \gamma + \Bigl(1+\gamma\tfrac{2\mon}{1+\theta}\Bigr)\tfrac{\com}{\theta} > 0
%                 {}\stackrel{\theta\,>\,0}{\Longleftrightarrow}{}
%             \Bigl(2\theta + \tfrac{4\mon\com}{1+\theta}\Bigr)\gamma + 2\com > 0
%             % \Bigl(\theta + \tfrac{2\mon\com}{1+\theta}\Bigr)\gamma + \com > 0
%                 {}\Leftrightarrow{}
%             (1 + \theta)\gamma + 2\com > 0
%             %     {}\Longleftrightarrow{}
%             % \gamma > -\tfrac{2\com}{1 + \theta}
%         \end{align*}
%         which is satisfied as $\gamma >  -\tfrac{2\com}{1+\theta}$ by \Cref{tab:semimon:domain}.
%         Denote 
%         \(
%             \hat A \coloneqq (A-\nu \id)^{-1} + \omega \id
%         \). 
%         % First, we will show that \(\omega + \tfrac{1}{\theta} > 0\)  
%         Owing to \(\omega + \xi > 0\) and Minty's theorem \cite[Thm. 21.1]{bauschke2017Convex}, the operator 
%         \[
%             \tfrac{1}{\omega+\xi}\hat A 
%                 {}={}
%             \tfrac{1}{\omega+\xi}
%             \left(%
%                 (A-\nu\id)^{-1} - \xi\id
%             \right)
%                 {}+{}
%             \id
%         \] 
%         has full range iff \(\tfrac{1}{\omega+\xi}\big((A-\nu\id)^{-1} - \xi\id\big)\) is maximally monotone. This along with \(\omega+\xi>0\) and \cref{cor:generation semimonotone operator} implies that \(A\) is maximally semimonotone iff \(\hat A\) has full range. Therefore, it suffices to show that the later condition is equivalent to \(\range{\id+\gamma A}=\R^n\), \ie, that the resolvent has full domain. 

%         First assume that \(\hat A\) has full range. Fix \(y\in\R^n\). By the full range assumption for \(\hat A\), there exists some \(x\in\R^n\) such that 
%         \(
%             \tfrac{\omega}{\gamma} y\in (A - \nu \id)^{-1}x+\omega x.
%         \) 
%         Letting \(z = \omega(\tfrac{1}{\gamma}y-x)\) we have 
%         \begin{align*}
%             \tfrac{1}{\gamma} y - \tfrac1{\omega}z \in (A - \nu \id)z  
%                 {}\iff{}
%             \tfrac{1}{\gamma} y \in \big(A + (\tfrac1{\omega} - \nu) \id\big)z      
%                 {}\iff{}
%             y \in \big(\gamma A +  \id\big)z,    
%             \numberthis\label{eq:semimon:resolvent:1}  
%         \end{align*}
%         where in the last equivalent we used the fact that \(\gamma = \tfrac{\omega}{1-\omega \nu}\). Since the choice of \(y\) was arbitrary, \(J_{\gamma A}\) has full domain. 
        
%         The converse follows similarly. Assume that  \(\range{\I+\gamma A}=\R^n\). For any fixed \(y\in\R^n\) there exists some \(z\in\R^n\) such that \(y\in \gamma Az + z\). Therefore, by \eqref{eq:semimon:resolvent:1} and letting \(x = \tfrac{1}{\gamma}y - \tfrac{1}{\omega}z\) we obtain \(\tfrac{\omega}{\gamma}y\in\hat Ax\), thus establishing that \(\range{\hat A}=\R^n\).  
%     \end{proofitemize}
%     \end{proofitemize}
%     \vspace*{-10pt}
%     \[\] % to fix SIAM's qed bug
% \end{appendixproof}


    % We begin by showing that \((A-\nu \id)^{-1}-\xi \id\) is maximally monotone iff the operator \(\hat A\) has full range.  

    % From \cref{cor:generation semimonotone operator} the operator \((A-\nu \id)^{-1}-\xi \id\) is maximally monotone. Let 
    
    % Owing to the assumption \(\omega+ \xi>0\), by Minty's theorem \cite[Thm. 21.1]{bauschke2017Convex}, the operator 
    % \[
    %     \tfrac{1}{\omega+\xi}\hat A 
    %         {}={}
    %     \tfrac{1}{\omega+\xi}
    %     \left(%
    %         (A-\nu\id)^{-1} - \xi\id
    %     \right)
    %         {}+{}
    %     \id
    % \] 
    % has full range, in turn implying the same for \(\hat A\).  
    % % Thus, by Minty's theorem \cite[Thm. 21.1]{bauschke2017Convex} the operator 
    % % \(
    % %     \hat A \coloneqq (T-\nu \id)^{-1} + \omega \id
    % % \)
    % % has full range since we assumed
    % % % \(\gamma \in (-\tfrac{\xi}{1+\nu\xi}, -\tfrac{1}{\nu})\) which implies 
    % % \(\omega > -\xi\). 
    % Fix \(y\in\R^n\). Since \(\hat A\) has full range, there exists some \(x\in\R^n\) such that 
    % \(
    %     \tfrac{\omega}{\gamma} y\in (A - \nu \id)^{-1}x+\omega x.
    % \) 
    % Letting \(z = \omega(\tfrac{1}{\gamma}y-x)\) we have 
    % \begin{align*}
    %     \tfrac{1}{\gamma} y - \tfrac1{\omega}z \in (A - \nu \id)z  
    %         {}\iff{}
    %     \tfrac{1}{\gamma} y \in \big(A + (\tfrac1{\omega} - \nu) \id\big)z      
    %         {}\iff{}
    %     y \in \big(\gamma A +  \id\big)z,      
    % \end{align*}
    % where in the last equivalent we used the fact that \(\gamma = \tfrac{\omega}{1-\omega \nu}\). Since the choice of \(y\) was arbitrary, \(J_{\gamma A}\) has full domain. 

    
  

    % Take $(u,x), (v, y) \in \gph J_{\gamma A}$. It remains to prove that
    % \begin{equation}\label{eq:cor:semimon:lipschitz}
    %     \nrm{x-y} \leq L(\gamma)\nrm{u-v}.
    % \end{equation}
    % First, note that $\gamma^{-1}(u-x) \in Tx$ and $\gamma^{-1}(v-y) \in Ty$, such that due to semimonotonicity of $A$ it holds that
    % \begin{align*}
    %     \mon \nrm{x-y}^2 + \com \gamma^{-2} \nrm{(u-v)-(x-y)}^2 &\leq \inner{\gamma^{-1}(u-x) - \gamma^{-1}(v-y), x-y}\\
    %     & = \gamma^{-1}\inner{u-v, x-y} - \gamma^{-1}\nrm{x-y}.
    % \end{align*}
    % Expanding the last term in the left-hand side and rearranging, we get
    % \begin{equation}\label{eq:cor:semimon:inequality}
    %     \begin{aligned}
    %         \left(1 + \mon\gamma + \com \gamma^{-1}\right)\nrm{x-y}^2 + \com \gamma^{-1}\nrm{u-v}^2 &\leq \left(1 + 2 \com \gamma^{-1}\right)\inner{u-v,x-y}\\
    %         & \leq \left|1 + 2 \com \gamma^{-1}\right|\nrm{u-v}\nrm{x-y}.
    %     \end{aligned}
    % \end{equation}
    % From \eqref{eq:semimon:fulldom:gamma} follows that \(1 + \mon\gamma + \com \gamma^{-1} > 0\). Hence, if \(u=v\) then necessarily \(x=y\) and thus \eqref{eq:cor:semimon:lipschitz} holds. Otherwise, define
    % \[
    %     \omega \dfn \tfrac{\nrm{x-y}}{\nrm{u-v}}    
    % \]
    % such that \eqref{eq:cor:semimon:inequality} is equivalent to
    % \begin{equation*}
    %         \left(1 + \mon\gamma + \com \gamma^{-1}\right)\omega^2 - \left|1 + 2 \com \gamma^{-1}\right| \omega + \com \gamma^{-1} \leq 0.
    % \end{equation*}
    % Solving this quadratic inequality for $\omega$, we directly obtain that \eqref{eq:cor:semimon:lipschitz} holds, which concludes the proof.



==> TeX/Text/Proofs/SemiMonInverse.tex <==
%!TEX root = ../../../CP-Minty.tex

% \begin{appendixproof}{prop:calculus:inverse}
%     On the one hand, if $A$ is $(\Mon,\Com)$\hyp{}semimonotone at $(\other{x}, \other{y})$, then \cref{eq:obliquequasisemimonotonicity:matrix} holds $\forall (x, y) \in \gph A$. Hence, we equivalently have that \cref{eq:obliquequasisemimonotonicity:matrix} holds $\forall (y, x) \in \gph A^{-1}$, and thus $A^{-1}$ is $(\Com, \Mon)$\hyp{}semimonotone at $(\other{y}, \other{x})$.
%     On the other hand, if $A^{-1}$ is $(\Com, \Mon)$\hyp{}semimonotone at $(\other{y}, \other{x})$, then \cref{eq:obliquequasisemimonotonicity:matrix} holds $\forall (x, y) \in \gph A^{-1}$. Hence, we equivalently have that \cref{eq:obliquequasisemimonotonicity:matrix} holds $\forall (y, x) \in \gph A$, and thus $A$ is $(\Mon, \Com)$\hyp{}semimonotone at $(\other{x},\other{y})$. The argument for (maximally) semimonotone operators is analogous. 
% \end{appendixproof}

==> TeX/Text/Unused/Rosenbrock.tex <==

TODO: rework and add text. This would be our second example
% \begin{example}[Rosenbrock function]\label{ex:Rosenbrock}
%     Let $b > 0$ and let $g : \R \rightarrow \Rinf$ be a proper lower semicontinuous function satisfying 
%     \[
%         g(0) = 0,
%         \quad
%         0 \in \partial g(0)
%         \quad\text{and}\quad
%         g(y) \geq \tfrac14y^2
%         \quad\text{for all}\quad
%         y \in \R.
%     \]
%     Consider the minimization problem
%     \begin{align*}
%         \minimize_{x \in \R^3}
%         \quad
%         \underbrace{
%         x_1x_2
%             +
%         b(x_3-x_1^2)^2
%         }_{\eqqcolon f(x)}
%             +
%         g(Lx)
%         \quad
%             \text{where}
%         \quad
%         L
%             \coloneqq
%         \begin{bmatrix}
%             1 & -1 & 0
%         \end{bmatrix}.
%         \numberthis\label{eq:ex:Rosenbrock}
%     \end{align*}
%     Then, the following hold.
%     \begin{enumerate}
%         \item The global minimum of \eqref{eq:ex:Rosenbrock} is given by $x^\star = (0, 0, 0)$.
%         \item $\nabla f$ is 
%         $\Bigl(-\nicefrac98 L^\top L, -\nicefrac{1}{4}\proj_{\ker{L}}\Bigr)$-semimonotone
%         at $(x^\star, 0)$.
%     \end{enumerate}
%     Suppose that 
%     $\partial g$ is $(3, 0)$-semimonotone at $(Lx^\star, 0) = (0,0)$. Then,
%     \begin{enumerate}
%         \item        
%         The pair
%         \((x^\star, 0) \in \zer \Tpd\)
%         is a $\DRSRho$\hyp{}oblique weak Minty solution of $\Tpd$
%         with $\DRSRho$ given by \eqref{eq:WMSDRS}, where 
%         $
%             \DRSrhocom = 0,
%             \DRSrhomon = -\nicefrac{9}{5},
%             \DRSrhocom^\prime = -\nicefrac14
%         $
%         and
%         $
%             \DRSrhomon^\prime = 0
%         $.
%         \item
%         The sequence $\seq{z^k} = \seq{x^k,y^k}$ generated by \ref{eq:CP} with fixed relaxation parameter $\lambda$ converges for 
%         $
%             \gamma \in 
%             \Bigl(\nicefrac14, \nicefrac5{18}\Bigr),
%             \tau \in 
%             \Bigl(\nicefrac{9}{5}, \nicefrac{1}{2\gamma}\Bigr]
%         $
%         and 
%         $
%             \lambda \in (0, 2 - \tfrac{6}{\tau}).
%         $
%         \qedhere
%     \end{enumerate}
% \end{example}
\begin{example}[Rosenbrock function]\label{ex:Rosenbrock}
    Let $b > 0$ and $\mon > \nicefrac{18}{7}$.
    Let
    $
        g(\cdot) \coloneqq \tfrac{\mon}{2}\|\cdot\|^2
    $,
    which includes the case
    $
        g = \delta_{\set{0}}
    $
    as a special case by letting $\mon$ go to $+\infty$.
    % Let $b > 0$ and let $g : \R \rightarrow \Rinf$ be a proper lower semicontinuous function satisfying 
    % \[
    %     g(0) = 0,
    %     \quad
    %     0 \in \partial g(0)
    %     \quad\text{and}\quad
    %     g(y) \geq \tfrac14y^2
    %     \quad\text{for all}\quad
    %     y \in \R.
    % \]
    Consider the minimization problem
    \begin{align*}
        \minimize_{x \in \R^3}
        \quad
        \underbrace{
        x_1x_2
            +
        b(x_3-x_1^2)^2
        }_{\eqqcolon f(x)}
            +
        g(Lx)
        \quad
            \text{where}
        \quad
        L
            \coloneqq
        \begin{bmatrix}
            1 & -1 & 0
        \end{bmatrix}.
        \numberthis\label{eq:ex:Rosenbrock}
    \end{align*}
    Then, the following hold.
    \begin{enumerate}
        \item The global minimum of \eqref{eq:ex:Rosenbrock} is given by $x^\star = (0, 0, 0)$.
        \item $\nabla f$ is 
        $\Bigl(-\nicefrac98 L^\top L, -\nicefrac{1}{4}\proj_{\ker{L}}\Bigr)$-semimonotone
        at $(x^\star, 0)$ and
        $\partial g$ is $(\mon, 0)$-semimonotone at $(Lx^\star, 0) = (0,0)$.
        \item        
        The pair \((x^\star, 0) \in \zer \Tpd\)
        is a $\DRSRho$\hyp{}oblique weak Minty solution of $\Tpd$
        with $\DRSRho$ given by \eqref{eq:WMSDRS}, where 
        $
            \DRSrhocom = 0,
            % \DRSrhomon = -\nicefrac{9}{5},
            \DRSrhomon = \nicefrac{9\mon}{(9 - 8\mon)},
            \DRSrhomon = -\nicefrac{9}{5},
            \DRSrhocom^\prime = -\nicefrac14
        $
        and
        $
            \DRSrhomon^\prime = 0
        $.
        \item
        The sequence $\seq{z^k} = \seq{x^k,y^k}$ generated by \ref{eq:CP} with fixed relaxation parameter $\lambda$ converges for 
        \[
            \gamma \in 
            % \Bigl(\nicefrac14, \nicefrac5{18}\Bigr),
            \Bigl(\nicefrac14, \nicefrac{(8\mon - 9)}{18\mon}\Bigr),
            \;
            \tau \in 
            % \Bigl(\nicefrac{9}{5}, \nicefrac{1}{2\gamma}\Bigr]
            \Bigl(\nicefrac{9\mon}{(8\mon - 9)}, \nicefrac{1}{2\gamma}\Bigr]
            \;\text{and}\;
            \lambda \in \Bigl(0, 2\left(1 + \min\left\{\nicefrac{9\mon}{(9 - 8\mon)\tau}, -\nicefrac{1}{4\gamma}\right\}\right)\Bigr).
        \]
        \qedhere
    \end{enumerate}
    \begin{proof}
        \hl{TODO}
    \end{proof}
\end{example}

==> TeX/Text/Unused/comment_singleton.tex <==
    As a further remark, note also that if $x^0 \in \R^n$ and $y^0 \in \R^m$ are selected such that
    \(
        x^0 - \gamma L^\top y^0 \in \dom J_{\gamma A}
    \)
    and
    \(
        y^0 + \tau L(2\bar x^0 - x^0) \in \dom_{\tau B^{-1}}
    \),
    then leveraging \eqref{eq:cor:CP:semi:singleton:resA} and \eqref{eq:cor:CP:semi:singleton:resB} it follows by construction that $\bar z^0 = (\bar x^0, \bar y^0) \in \zer \Tpd$ and thus the algorithm reaches a solution in a single iteration.

==> TeX/Text/Unused/general_quadratic.tex <==
As an implication of \Cref{thm:calculus:primaldual}, consider the following result for the primal-dual operator emerging in constrained QP problems.

\begin{example}[constrained QP]\label{ex:constrainedQP}
    Consider the quadratic program
    \begin{align*}
        \minimize_{x\in\R^n} \quad \tfrac12 x^\top Q x + q^\top x\quad
        \stt \quad L x \in C,\numberthis\label{eq:QP}
    \end{align*}
    where 
    $Q \in \sym{n}$, $q \in \R^n$. $L \in \R^{m \times n}$ and $C \dfn \set{x\in \R^m}[l_i \leq x_i \leq u_i, \; i = 1, \dots, m]$, where $l, u \in \R^m$.
    The associated first-order optimality condition is given by
    $
        0 \in Ax + L^\top B L x,
    $
    where $A : x \mapsto Qx + q$ and $B \dfn N_{C}$. 
    Suppose that
    $L$ is full column rank or that
    $
        \proj_{\range{L^\top}} Q \proj_{\ker{L}} = 0
    $
    and
    $
        \proj_{\ker{L}} Q \proj_{\ker{L}} \succeq 0
    $.
    Then, the following assertions hold.
    \begin{enumerate}
        \item \label{it:QP:A:full} Operator $A$ is $(L^\top \MonA L, \ComA^\prime)$
        % = (\proj_{\rge{L^\top}}Q\proj_{\rge{L^\top}}, Q^\dagger - Q^\dagger \proj_{\rge{L^\top}}Q \proj_{\rge{L^\top}} Q^\dagger)$
        -semimonotone, where 
        $\MonA = {L^\dagger}^\top Q L^\dagger$
        and
        $
            \ComA^\prime = \proj_{\ker{L}} Q^\dagger \proj_{\ker{L}}
        $.
        \item \label{it:QP:B:box} 
        Let
        $
            (x^\star, y^\star) 
            %     = 
            % (x^\star, -{L^\dagger}^\top A x^\star) 
                \in
            \zer \Tpd
        $
        and
        $
            \MonB
                \coloneqq
            \diag\Bigl(\frac{|y^\star_1|}{u_1 - l_1}, \dots, \frac{|y^\star_n|}{u_n - l_n}\Bigr)
        $.
        Then, operator $B$ is $\Bigl(\MonB, 0\Bigr)$-semimonotone at $(Lx^\star, y^\star) \in \gph B$.
        \item \label{it:QP:Tpd}
        % The primal-dual operator 
        If there exists a primal-dual pair
        $
            (x^\star, y^\star) 
            %     = 
            % (x^\star, -{L^\dagger}^\top A x^\star) 
                \in
            \zer \Tpd
        $
        satisfying
        % all points \((x^\star, y^\star) = (x^\star, -{L^\dagger}^\top A x^\star) \in \R^{n+m}\) such that 
        \(
            % (Lx^\star, y^\star) \in \gph B
            % \quad\text{and}\quad
            \left(
                % {L^\dagger}^\top Q L^\dagger, 
                \MonA,
                % \diag\left(\frac{|y^\star_1|}{u_1 - l_1}, \dots, \frac{|y^\star_n|}{u_n - l_n}\right)
                \MonB
            \right) \in \parsumset,
            % \numberthis\label{eq:QP:WMVI:cond}
        \)
        then \Cref{ass:SWMVICP} is satisfied
        % is a $\DRSRho$\hyp{}oblique weak Minty solution of $\Tpd$
        % with $\DRSRho$ given by \eqref{eq:WMSDRS}, where 
        for
        \(
            \DRSrhocom = 0
        \),
        \(
            \DRSrhomon = \lambda_{\rm min}\left(\UL^\top\left(
                % {L^\dagger}^\top Q L^\dagger 
                \MonA
                \Box 
                % \diag\left(\frac{|y^\star_1|}{u_1 - l_1}, \dots, \frac{|y^\star_n|}{u_n - l_n}\right)
                \MonB
            \right)\UL\right)
        \),
        \(
            \DRSrhomon^\prime = 0
        \)
        and
        \(     
            \DRSrhocom^\prime 
                {}={}
            \lambda_{\rm min}\Bigl({\VL'}^\top
                    % Q^\dagger - Q^\dagger \proj_{\rge{L^\top}} Q \proj_{\rge{L^\top}} Q^\dagger
                    Q^\dagger
                \VL'\Bigr) \geq 0.
        \)
        % In numerical experiments, this seems to hold at the zeros of Tpd when $0 \notin C$. (i.e. the 'top' of the quadratic is not located inside the box)
    \end{enumerate}

    \begin{proof}
        \begin{proofitemize}
            \item \ref{it:QP:A:full}: 
            Let $\Mon \dfn L^\top \MonA L = \proj_{\rge{L^\top}} Q \proj_{\rge{L^\top}}$ and observe that
            \begin{align*}
                \proj_{\ker{Q}} \Mon
                    {}={}
                \proj_{\ker{Q}} \proj_{\rge{L^\top}} Q \proj_{\rge{L^\top}}
                    {}={}
                \proj_{\ker{Q}} (\I_n - \proj_{\ker{L}}) Q \proj_{\rge{L^\top}}
                    {}={}
                0,
                \numberthis\label{eq:proof:ex:constrainedQP:projQ-M}
            \end{align*}
            where the final equality holds since $\proj_{\range{L^\top}} Q \proj_{\ker{L}} = 0$.
            Therefore, \eqref{eq:LMI:condition:lin} is satisfied for $D = Q$ and $Q$ is $(L^\top \MonA L, \Com^\star)$\hyp{}semimonotone by \Cref{prop:semi:lin:optimal}, where
            \(
                \Com^\star 
                    {}={}
                Q^\dagger - Q^\dagger \Mon Q^\dagger
                    {}={}
                Q^\dagger - Q^\dagger \proj_{\rge{L^\top}}Q \proj_{\rge{L^\top}} Q^\dagger
            \)
            owing to \eqref{eq:proof:ex:constrainedQP:projQ-M} and symmetry of $Q$.
            Moreover, since
            $
                \proj_{\range{L^\top}} Q \proj_{\ker{L}} = 0,
            $
            it holds owing to \cite[Fact 6.4.34]{bernstein2009matrix} that
            $
                Q^\dagger = (\proj_{\range{L^\top}} Q \proj_{\range{L^\top}})^\dagger + (\proj_{\ker{L}} Q \proj_{\ker{L}})^\dagger
            $,
            so that 
            $
                \Com^\star
                    {}={}
                \proj_{\ker{L}} Q^\dagger \proj_{\ker{L}}
                    {}={}
                \ComA^\prime
            $.
            The claimed result for $A : x \mapsto Qx + q$ then follows from \Cref{lem:calculus:scaling}.
            \item \ref{it:QP:B:box}: Owing to \Cref{prop:auslender}, it holds that $(x^\star, y^\star) \in \zer \Tpd$ if and only if $(x^\star, -L^\top y^\star) \in \gph A$ and $(L x^\star, y^\star) \in \gph B$. The claimed result then follows directly from \Cref{prop:box}.
            \item \ref{it:QP:Tpd}: 
            By \Cref{thm:calculus:primaldual}, $\Tpd$
            has
            $((\proj_{\ker{L}} Q^\dagger \proj_{\ker{L}}) \oplus (\MonA \Box \MonB))$\hyp{}oblique weak Minty solutions at $\pazocal{S}^\star = \set{(x^\star, y^\star)}$.
            Therefore, using that $\proj_{\ker{L}} = \VL^\prime {\VL^\prime}^\top$, it follows that the parameters $\DRSrhocom, \DRSrhomon, \DRSrhocom'$ and $\DRSrhomon'$ given in \ref{it:QP:Tpd} match those from \eqref{eq:calculus:primaldual:params}.
            As remarked below \Cref{thm:calculus:primaldual}, \Cref{ass:SWMVICP} holds since these parameters satisfy condition \eqref{eq:existence:condition}, completing the proof.
            \qedhere
        \end{proofitemize}
    \end{proof}
\end{example}
Leveraging this result, one can easily verify the underlying assumptions for \Cref{thm:CP:full}, i.e., \Cref{ass:CP}, for (nonconvex) quadratic programs.
For instance, consider the following numerical example, where \Cref{thm:CP:full} is applied to a nonconvex QP with an indefinite $Q$ matrix where $L$ is full row rank.
An example where $L$ is rank-deficient is provided later in \Cref{ex:constrainedQP:semi}.
% For instance, consider the convergence of \ref{eq:CP} for the following QP.
% where $L$ is full row rank and $\proj_{\rge{L^\top}} Q \proj_{\rge{L^\top}}$ is indefinite. In this setting, the semimonotonicity matrices of $A$ and $B$ are diagonal matrices, able to accurately capture the behavior of $A$ and $B$ along the different coordinates. 
% it can be seen that the diagonal structre o accurately capture the behavior of $A$ and $B$ along the different coordinate vectors. 
\begin{example}\label{ex:constrainedQP:Semi}
    \ifjota
        Consider the following quadratic program
        \begin{align*}
            \smash{\minimize_{x\in\R^n}} \quad \tfrac12 x^\top Q x + q^\top x\quad
            \stt \quad L x \in C,\numberthis\label{eq:QP}
        \end{align*}
        where 
    \else
        Let
    \fi
    $
        Q
            {}={}
        % \begin{bmatrix}
        %     1 & 0 & 0\\
        %     0 & -1 & 0\\
        %     0 & 0 & 2
        % \end{bmatrix}
        \diag(1, -1, 2)
    $,
    $
        q
            {}={}
        \begin{bsmallmatrix}
            -1&
            1&
            -1
        \end{bsmallmatrix}^\top
    $,
    $
        L = 
        \begin{bsmallmatrix}
            1 & \frac14 & 0\\
            0 & 1 & 0
        \end{bsmallmatrix}
    $
    and
    $
        C \dfn \set{x\in \R^2}[2 \leq x_i \leq 4, i = 1, 2]
    $\ifjota
        .
    \else
        \ in \Cref{ex:constrainedQP}.
    \fi
    \ifjota
        Then, the associated first-order optimality conditions are given by
        $
            0 \in Ax + L^\top B L x,
        $
        where $A : x \mapsto Qx + q$ and $B \dfn N_{C}$, and the global minimizer of \eqref{eq:QP} is given by         
        $
            x^\star 
                = 
            \begin{bsmallmatrix}
                1 &
                4 &
                \frac12
            \end{bsmallmatrix}^\top
        $.
        The following assertions hold.
    \else
        Then, the global minimizer is given by
        $
            x^\star 
                = 
            \begin{bsmallmatrix}
                1 &
                4 &
                \frac12
            \end{bsmallmatrix}^\top
        $
        and the following assertions hold.
    \fi
    \begin{enumerate}
        \item \label{it:QP:A:full:Semi} 
        \ifjota\else
            Operator 
        \fi
        $A$ is 
        $
            \bigl(\diag(1, -1, 0), \diag(0,0,\tfrac12)\bigr)
        $\hyp{}semimonotone.
        \item 
        \ifjota\else
            Operator 
        \fi
        $B$ is 
        $
            \bigl(\diag(0, \tfrac32), 0\bigr)
        $\hyp{}semimonotone at 
        $
            (Lx^\star, -{L^\dagger}^\top A x^\star) 
                = 
            \left(
                \begin{bsmallmatrix}
                    2 \\
                    4
                \end{bsmallmatrix}
                , 
                \begin{bsmallmatrix}
                    0 \\
                    3
                \end{bsmallmatrix}
            \right) 
            \in \gph B
        $.
        \item \label{it:QP:Tpd:Semi}
        The
        \ifjota\else
            primal-dual
        \fi
        pair
        \((x^\star, -{L^\dagger}^\top A x^\star) \in \zer \Tpd\)
        is a $\DRSRho$\hyp{}oblique weak Minty solution of $\Tpd$
        with $\DRSRho$ given by \eqref{eq:WMSDRS}, where 
        $
            \DRSrhocom = 0,
            \DRSrhomon = -3,
            \DRSrhocom^\prime = \tfrac12
        $
        and
        $
            \DRSrhomon^\prime = 0
        $
        as in \eqref{eq:calculus:primaldual:params}.
        \item \label{it:QP:CP:Semi}
        The sequence $\seq{z^k} = \seq{x^k,y^k}$ generated by \ref{eq:CP} with fixed relaxation parameter $\lambda$ converges for 
        \ifjota
            $
                \gamma \in 
                % \bigl(0, \tfrac{-1}{\DRSrhomon\nrm{L}^2}\bigr) \approx 
                (0, 0.26),
                \tau \in 
                % \bigl(-\DRSrhomon, \tfrac{1}{\gamma\nrm{L}^2}\bigr] \approx 
                (3, \tfrac{0.779}{\gamma}]
            $
            and 
            $
                \lambda \in 
                % (0, 2 + \tfrac{2}{\tau} \DRSrhomon) = 
                (0, 2 - \tfrac{6}{\tau}).
            $
        \else
            $$
                \gamma \in \Bigl(0, \tfrac{-1}{\DRSrhomon\nrm{L}^2}\Bigr) \approx (0, 0.26),
                \quad
                \tau \in \Bigl(-\DRSrhomon, \tfrac{1}{\gamma\nrm{L}^2}\Bigr] \approx (3, \tfrac{0.779}{\gamma}],
                \quad
                \lambda \in (0, 2 + \tfrac{2}{\tau} \DRSrhomon) = (0, 2 - \tfrac{6}{\tau}),
            $$
            where we used that $\nrm{L}^2 = \tfrac{33 + \sqrt{65}}{32} \approx 1.28$. \qedhere
        \fi
    \end{enumerate}
    \begin{proof}
        \ifjota
            The different assertions follow from \Cref{prop:semi:lin}, \cite[Prop. A.5]{evens2023convergenceCP}, \Cref{thm:calculus:primaldual} and \Cref{thm:CP:full}, respectively.
        \else
            The claimed assertions follow from those of \Cref{ex:constrainedQP}
            and \Cref{thm:CP:full},
            using that 
            $
                L^\dagger = 
                % \begin{bsmallmatrix}
                %     1 & -1/4\\
                %     0 & 1\\
                %     0 & 0
                % \end{bsmallmatrix}           
                \begin{bsmallmatrix}
                    1 & 0 & 0\\
                    -\frac14 & 1 & 0
                \end{bsmallmatrix}^\top
            $,
            $
                \proj_{\rge{L^\top}} = \diag(1, 1, 0)
            $,
            $
                \MonA = 
                \tfrac{1}{16}
                \begin{bsmallmatrix}
                    16 & -4\\
                    -4 & -15
                \end{bsmallmatrix}
            $,
            $
                \MonA \Box \diag(0, \tfrac32) = \diag(0, -3)
            $
            and continuity of $J_{\gamma A}$ and $J_{\tau B^{-1}}$.
        \fi
    \end{proof}
\end{example}

\Cref{cor:CP:semi} provides a set of sufficient conditions for the convergence of \ref{eq:CP} which can be easily verified based on the calculus rules for semimonotone operators developed in \Cref{sec:semi} and \cite[Sec. 4]{evens2023convergence}. To demonstrate this, \Cref{cor:CP:semi} will be applied to several examples previously discussed in this paper.

First of all, consider the following constrained QP, where $Q$ is an indefinite matrix and $L$ is rank-deficient. Previously, it was shown for the nonconvex QP from \Cref{ex:constrainedQP:Semi} that convergence of \ref{eq:CP} can be established using \Cref{thm:calculus:primaldual} and \Cref{thm:CP:full}. 
In this example, we show that if the monotonicity of $A$ can be expressed in the form $\monA L^\top L$, then this result can be obtained directly using \Cref{cor:CP:semi}.
% Note that in this example, $Q$ is an indefinite matrix and $L$ is rank-deficient.
% First of all, consider the following particular instance of \Cref{ex:constrainedQP}, where $Q$ is an indefinite matrix and $L$ is rank-deficient. 

\begin{example}\label{ex:constrainedQP:semi}
    Consider the QP from 
    \ifjota
        \Cref{ex:constrainedQP:Semi},
    \else
        \Cref{ex:constrainedQP},
    \fi
    where
    $
        Q
            {}={}
        \diag(-3, -2, 1)
    $,
    $
        q
            {}={}
        \begin{bsmallmatrix}
            0&
            1&
            0
        \end{bsmallmatrix}^\top
    $,
    $
        L = 
        \begin{bsmallmatrix}
            1 & 0 & 0\\
            1 & 1 & 0\\
            1 & -1 & 0
        \end{bsmallmatrix}
    $
    and
    $
        C \dfn \set{x\in \R^2}[\nicefrac12 \leq x_i \leq 1, \; i = 1, 2, 3].
    $
    Then, the global minimizer is given by         
    $
        x^\star 
            = 
        \begin{bsmallmatrix}
            1 &
            0 &
            0
        \end{bsmallmatrix}^\top
    $
    and the following assertions hold.
    \begin{enumerate}
        \item 
        \ifjota\else
            Operator 
        \fi
        $A$ is 
        \ifjota
            $
                \bigl(-L^\top L, \diag(0,0,1)\bigr)
            $\hyp{}semimonotone.
        \else
            $
                \bigl(\monA L^\top L, \diag(0,0,1)\bigr)
            $\hyp{}semimonotone where $\monA = -1$.
        \fi
        \item 
        \ifjota\else
            Operator 
        \fi
        $B$ is 
        \ifjota
            $
                \bigl(2\I, 0\bigr)
            $%
        \else
            $
                \bigl(\monB\I, 0\bigr)
            $%
        \fi
        \hyp{}semimonotone at 
        $
            (Lx^\star, -{L^\dagger}^\top A x^\star) 
                = 
            \left(
                \begin{bsmallmatrix}
                    1 &
                    1 &
                    1
                \end{bsmallmatrix}^\top
                , 
                \begin{bsmallmatrix}
                    1 &
                    1 &
                    1
                \end{bsmallmatrix}^\top
            \right) 
            \in \gph B
        $\ifjota.
        \else
            \ where $\monB = 2$.
        \fi
        % \item 
        % The primal-dual pair 
        % \((x^\star, -{L^\dagger}^\top A x^\star) \in \zer \Tpd\)
        % is a $\DRSRho$\hyp{}oblique weak Minty solution of $\Tpd$
        % with $\DRSRho$ given by \eqref{eq:WMSDRS}, where 
        % \begin{align*}
        %     \DRSrhocom = 0,
        %     \quad
        %     \DRSrhomon
        %     %  = \lambda_{\rm min}
        %     % \Bigl(
        %     %     \tfrac{1}{440}
        %     %     \begin{bmatrix}
        %     %         144 & -68 \\
        %     %         -68 & -799
        %     %     \end{bmatrix}
        %     % \Bigr),
        %         = 
        %     -1 \Box 2 = -2,
        %     \quad
        %     \DRSrhocom^\prime = 0,
        %     \quad
        %     \DRSrhomon^\prime = 0,
        % \end{align*}
        \item The sequence $\seq{z^k} = \seq{x^k,y^k}$ generated by \ref{eq:CP} with fixed relaxation parameter $\lambda$ converges for 
        \ifjota
            $
                \gamma \in 
                % \bigl(0, \tfrac{-1}{(\monA \Box \monB)\nrm{L}^2}\bigr) = 
                (0, \tfrac16),
                \tau \in 
                % \bigl(-(\monA \Box \monB), \tfrac{1}{\gamma\nrm{L}^2}\bigr] =
                (2, \tfrac{1}{3\gamma}]
            $
            and
            $
                \lambda \in 
                % \bigl(0, 2 + \tfrac{2}{\tau} (\monA \Box \monB)\bigr) = 
                (0, 2 - \tfrac{4}{\tau}).\qedhere
            $
        \else
            $$
                \gamma \in \bigl(0, \tfrac{-1}{(\monA \Box \monB)\nrm{L}^2}\bigr) = (0, \tfrac16),
                \quad
                \tau \in \bigl(-(\monA \Box \monB), \tfrac{1}{\gamma\nrm{L}^2}\bigr] = (2, \tfrac{1}{3\gamma}],
                \quad
                \lambda \in \bigl(0, 2 + \tfrac{2}{\tau} (\monA \Box \monB)\bigr) = (0, 2 - \tfrac{4}{\tau}).\qedhere
            $$
        \fi
    \end{enumerate}
    \begin{proof}
        \ifjota
            The different assertions follow from \Cref{prop:semi:lin}, \cite[Prop. A.5]{evens2023convergenceCP} and \Cref{cor:CP:semi}, respectively.
        \else
            The claimed assertions follow from those of \Cref{ex:constrainedQP}
            and \Cref{cor:CP:semi},
            using that 
            $A$ is        
            $
                \bigl(\monA L^\top L, 0\bigr)
            $\hyp{}semimonotone,
            $
                L^\dagger = 
                \tfrac16         
                \begin{bsmallmatrix}
                    2 & 2 & 2\\
                    0 & 3 & -3\\
                    0 & 0 & 0
                \end{bsmallmatrix}
            $
            and continuity of $J_{\gamma A}$ and $J_{\tau B^{-1}}$.
        \fi
    \end{proof}
\end{example}

==> TeX/Text/Unused/linear.tex <==
%!TEX root = ../../../CP_WMVI.tex
In the following corollary, it is shown that despite presence of
nonmonotonicity, linear convergence of \eqref{eq:CP} is attained for
piecewise polyhedral operators. 

\begin{definition}[piecewise polyhedral mappings]
    A set-valued mapping \(T:\R^n\rightrightarrows\R^n\) is said to be piecewise polyhedral if its graph can be expressed as the union of finitely many polyhedral sets.
\end{definition}

The class of piecewise polyhedral mappings trivially include piecewise linear mappings, and the subgradient of all piecewise linear quadratic convex functions such as normal cones of polyhedral sets \cite[Sect. 12]{rockafellar2009Variational}. The proof of \Cref{cor:DRS:CP:lin} is similar to \cite[Lem. IV.4]{Latafat2019Randomized} and is included in the appendix for completeness.

\begin{theorem}[linear convergence for piecewise polyhedral mappings]
    \label{cor:DRS:CP:lin}
    Suppose that \(A\) and \(B\) are piecewise polyhedral mappings, that \(\zer \Tpd\) is nonempty closed convex, and that \cref{ass:SWMVICP} holds with \(\pazocal{S}^\star = \zer \Tpd\). Set the stepsizes \(\gamma, \tau\) according to \Cref{ass:CP:stepsize:rule} and suppose that the resolvents \(J_{\gamma A}\), \(J_{\tau B^{-1}}\) have full domain and are continuous. 
    % Let \(\lambda_k \in (0, 2\alpha)\) such that \(\varepsilon \coloneqq \inf_{k\geq 0} \lambda_k(2\alpha -\lambda_k) > 0\), where $\alpha$ is defined as in
    % \Cref{thm:pppaDRS}. Then, 
    % the sequences \(\seq{s^k}\), \(\seq{\|u^k-v^k\|}\) generated by \ref{eq:DRS} with stepsize $\gamma$ and relaxation parameters $\seq{\lambda_k}$ starting from $s^0 \in \R^n$ converge at \(R\)-linear rate. 
    Consider the sequences $\seq{z^k} = \seq{x^k,y^k}$ and $\seq{\z^k} = \seq{\x^k,\y^k}$ generated by \ref{eq:CP} starting from $z^0 = (x^0, y^0) \in \R^{n+m}$ with stepsizes $\gamma, \tau$
    and relaxation parameters $\lambda_k \in \left(0,2\etamin\right)$ such that \(\liminf_{k\rightarrow \infty} \lambda_k(2\etamin -\lambda_k) > 0\), where $\etamin$ is defined as in
    \Cref{thm:CP:full} if $\DRSrhocom$ and $\DRSrhomon$ are not both strictly positive and as in \Cref{thm:CP:full:positive} otherwise.
    Then, \(\seq{\projQ z^k}\) and \(\seq{\|\projQ z^k-\projQ\bar z^k\|}\) converge \(R\)-linearly to zero.

    % Suppose that \cref{ass:CP} holds where \(\pazocal{S}^\star = \zer \Tpd\) in \cref{ass:SWMVICP} and that \(A\), \(B\) are piecewise polyhedral.
    % % Furthermore, suppose that \(\lambda_k \in (\varepsilon, 2\alpha-\varepsilon)\) where $\alpha > 0$ and \(\varepsilon\in(0,2\alpha)\).
    % Then, if $\gamma, \tau$ are selected according to \Cref{ass:CP:stepsize:rule}
    %     and \(\seq{\lambda_k} \subset (0, 2\etamin)\) such that \(\varepsilon \coloneqq \inf_{k\geq 0} \lambda_k(2\etamin -\lambda_k) > 0\), where $\etamin$ is defined as in \Cref{thm:CP:full,thm:CP:full:positive},
    %     the sequences \(\seq{\projQ \z^k}\) and \(\seq{\|\projQ \z^k-\projQ\bar \z^k\|}\) generated by \eqref{eq:CP} converge at \(R\)-linear rate. \hl{TODO: work out projections? Specific cases?}
\end{theorem}

\begin{remark}[Douglas-Rachford splitting]
    Note that when $L = \I$ and $\gamma = \nicefrac1\tau$, 
    the sequences $\seq{\projQ z^k}$ and $\seq{\projQ z^k - \projQ \z^k}$ in \Cref{cor:DRS:CP:lin}
    may be replaced by $\seq{x^k - \gamma y^k}$ and $\seq{\nrm{x^k - \gamma y^k - \x^k + \gamma \y^k}}$, respectively. 
    Consequently, \Cref{cor:DRS:CP:lin} matches the result from \cite[Thm. 3.5]{evens2023convergence}.
\end{remark}

==> TeX/Text/Unused/polyhedral.tex <==
\begin{proposition}[normal cone of a bounded polyhedral set]\label{prop:simplex}
    Let $\other{x}^i \in \R^n$, $\forall i \in I \dfn \set{1, \dots, p}$, be $p$ unique points where $p \geq 2$ and define $C \dfn \conv\bigl(\{\other{x}^i\}_{i \in I}\bigr)$ as the convex hull of these points. 
    Then, the normal cone $N_C: \R^n \rightrightarrows \R^n$ is $(\mon, 0)$-semimonotone at $(\other{x}^i, \other{v}^i) \in \gph N_C$, $\forall i \in I$, where
    $$
        \mon = \min\left\{\frac{\inner{\other{x}^i - \other{x}^j, \other{v}^i}}{\nrm{\other{x}^i - \other{x}^j}^2}\right\}_{j \in I\backslash i} \geq 0.
    $$
    \begin{proof}
        By definition $N_C$ is $(\mon, 0)$-semimonotone at $(\other{x}^i, \other{v}^i) \in \gph N_C$ if and only if
        \begin{align*}
            \inner{\other{x}^i - x, \other{v}^i - v} \geq \mon \nrm{\other{x}^i - x}^2, \quad \forall (x, v) \in \gph N_C,\numberthis\label{eq:prop:simplex:semi}
        \end{align*}
        If $x = \other{x}^i$, then \eqref{eq:prop:simplex:semi} holds for all $\mon \in \R$. Otherwise, for $\mon$ satisfying \eqref{eq:prop:simplex:semi} it holds that
        \begin{align*}
            \mon = \inf_{\substack{(x, v) \in \gph N_C\\ x\neq \other{x}^i}} &\quad \frac{\inner{\other{x}^i - x, \other{v}^i - v}}{\nrm{\other{x}^i - x}^2}
            {}={}
            \overbracket{\inf_{x \in C\backslash\{\other{x}^i\}} \frac{\inner{\other{x}^i - x, \other{v}^i}}{\nrm{\other{x}^i - x}^2}}^{\text{(B)}}
            +
            \overbracket{\inf_{v \in N_C(x)} \frac{\inner{x - \other{x}^i, v}}{\nrm{\other{x}^i - x}^2}}^{=0}.
        \end{align*}
        Due to monotonicity of the normal cone operator and since \((\other{x}^i,0)\in \graph N_C\) the last term is always nonnegative. Consequently, the minimum is attained for $v = 0 \in N_C(x)$. 

        Let $C^\prime = \conv\bigl(\{\other{x}^j\}_{j \in I\backslash i}\bigr)$ and observe that $C\backslash\{\other{x}^i\} = \set{\theta \other{x}^i + (1-\theta)x}[x \in C^\prime, \theta \in [0,1)]$. Consequently, it follows that
        \begin{align*}
            \text{(B)} 
                {}={}&
            \inf_{\theta \in [0,1), x^\prime \in C^\prime} \; \frac{1-\theta}{(1-\theta)^2}\underbrace{\frac{\inner{\other{x}^i - x^\prime, \other{v}^i}}{\nrm{\other{x}^i - x^\prime}^2}}_{\geq\,0}
                {}={}
            \inf_{x^\prime \in C^\prime} \; f(x^\prime) \dfn \frac{\inner{\other{x}^i - x^\prime, \other{v}^i}}{\nrm{\other{x}^i - x^\prime}^2},
        \end{align*}
        where we used that $f(x^\prime) \geq 0$ for all $x^\prime \in C^\prime \subset C$ since $(\other{x}^i, \other{v}^i) \in \gph N_C$.
        Consider the superlevel sets $S_\alpha \dfn \set{x^\prime \in C^\prime}[f(x^\prime) \geq \alpha]$, where $\alpha \in \R$. If $\alpha < 0$, then $S_\alpha = C^\prime$, which is convex. If $\alpha \geq 0$, convexity of $S_\alpha$ follows immediately from the convexity of $\alpha\nrm{x^\prime - \other{x}^i} - \inner{\other{x}^i - x^\prime, \other{v}^i}$. Therefore, $f$ is quasiconcave \cite[Sec. 3.4.1]{boyd2004Convex} and attains its minimum at one of the vertices of $C^\prime$, completing the proof.
    \end{proof}
\end{proposition}

==> TeX/Text/Unused/unused_calculusrules.tex <==

\begin{corollary}\label{it:prop:semi:lin:2}
    If $A = \alpha \I_n$ for some $\alpha \in \R$, then $A$ is \(\left(\alpha(1-\epsilon\alpha), \epsilon\right)\)\hyp{}semimonotone for any $\epsilon \in \R$ satisfying $\epsilon \neq \tfrac{1}{2\alpha}$ if $\alpha < 0$.
    \begin{proof}
        Let \(\left(\mon, \com\right) = \left(\alpha(1-\epsilon\alpha), \epsilon\right)\). Notice that $\mon < 0$ and $\com < 0$ if $\alpha < 0$ and $\epsilon \in (\tfrac{1}{\alpha}, 0)$. Hence, to ensure that $\mon \com < \tfrac{1}{4}$ if $\mon < 0$ and $\com < 0$, we need that $\epsilon \neq \tfrac{1}{2\alpha}$ if $\alpha < 0$.
        From \Cref{it:prop:semi:lin:1} and using that $A = \alpha \I_n$, it follows that $A$ is \(\left(\mon, \com\right)\)\hyp{}semimonotone if and only if \(\alpha \geq \mon + \com \alpha^2\). As this inequality is satisfied when \(\left(\mon, \com\right) = \left(\alpha(1-\epsilon\alpha), \epsilon\right)\) for any $\epsilon \in \R$, the proof is completed.
    \end{proof}
\end{corollary}

\begin{lemma}
    Let operator $A : \R^n \rightrightarrows \R^n$ be $(\MonA,\ComA)$\hyp{}semimonotone \optional{at $(\other{x}_A, \other{v}_A) \in \gph A$} and let $\alpha \in \R\backslash\{0\}$ and $\epsilon \in \R$.
    If $(\ComA,\epsilon\I) \in \parsumset$, then $A + \alpha \I$ is $\left(\MonA+\alpha(1-\epsilon\alpha),\ComA \Box \epsilon\I\right)$\hyp{}semimonotone \optional{at $(\other{x}_A, \other{v}_A+\alpha \other{x}_A)$}.
    \begin{proof}
        This result immediately follows from \Cref{prop:calculus:sum} and \Cref{it:prop:semi:lin:2}.
    \end{proof}
\end{lemma}

\begin{lemma}
    Let $L:\R^n\to \R^m$ be a linear mapping and operator $B : \R^m \rightrightarrows \R^m$ be $(\MonB,\ComB)$\hyp{}semimonotone \optional{at $(\other{x}_B, \other{v}_B) \in \gph \B$}.
    If \(\proj_{\ker{L}}^\top \MonB \proj_{\ker{L}} \succeq 0\) \optional{and $\other{v}_B = L\tilde{v}_B$ for some $\tilde{v}_B \in \R^n$}, then there exist matrices \(\MonB^\prime, \ComB^\prime \in \sym{n}\) satisfying \(L \MonB^\prime L^\top \preceq \MonB\) and \(\ComB^\prime \preceq L^\top \ComB L\) such that $L^\top \rhd B \dfn (L^\top B^{-1} L)^{-1}$
        is $(\MonB^\prime,\ComB^\prime)$\hyp{}semimonotone [at $(L^\top \other{x}_B, \tilde{v}_B)$].
    \begin{proof}
        From \Cref{prop:calculus:inverse} we know that $B^{-1}$ is $(\ComB,\MonB)$\hyp{}semimonotone \optional{at $(\other{v}_B, \other{x}_B) \in \gph B^{-1}$}. Hence, by \Cref{lem:calculus:composition:1} it follows that $L^\top B^{-1} L$ is $(\ComB^\prime,\MonB^\prime)$\hyp{}semimonotone \optional{at $(\tilde{v}_B, L^\top \other{x}_B)$} with \(\MonB^\prime, \ComB^\prime \in \sym{n}\) provided that \(L \MonB^\prime L^\top \preceq \MonB\) and \(\ComB^\prime \preceq  L^\top \ComB L\). 
        The claimed result follows directly by applying \Cref{prop:calculus:inverse} again.
    \end{proof}
\end{lemma}
 
\begin{lemma}
    Let $L:\R^n\to \R^m$ be a linear mapping and operator $B : \R^m \rightrightarrows \R^m$ be $(\MonB,\ComB)$\hyp{}semimonotone \optional{at $(\other{x}_B, \other{v}_B) \in \gph \B$}.
    Let operator $A : \R^n \rightrightarrows \R^n$ be $(\MonA,\ComA)$\hyp{}semimonotone \optional{at $(\other{x}_A, \other{v}_A) \in \gph A$} and operator $B : \R^m \rightrightarrows \R^m$ be $(\MonB,\ComB)$\hyp{}semimonotone \optional{at $(\other{x}_B, \other{v}_B) \in \gph \B$}.
    Let $n=m$. If $(\MonA,\MonB) \in \parsumset$ \optional{and $\other{v} = \other{v}_A = \other{v}_B$}, then $A \Box B$ is $(\MonA \Box \MonB, \ComA+\ComB)$\hyp{}semimonotone \optional{at $(\other{x}_A+\other{x}_B, \other{v})$}.
    \begin{proof}
        This is an immediate consequence of the definition of the parallel sum, owing to \Cref{prop:calculus:inverse} and \Cref{prop:calculus:sum}. 
    \end{proof}
\end{lemma}


\begin{table}[tb]
    \centering
    %% \input{TeX/Tables/Summary.tex} %%
    % Format
    \footnotesize
    \renewcommand{\arraystretch}{1.2}%
    \setlength\tabcolsep{5pt}%
    \newcommand{\header}[1]{\mc{1}{@{}c@{}}{\bf #1}}%
    \newcommand{\EITHER}{either~~\ignorespaces}%
    \newcommand{\OR}{\fillwidthof[r]{either}{or}~~\ignorespaces}%
    % Command shortcuts
        \let\mc\multicolumn%
        \newcommand{\mr}[2][2]{\multirow{#1}{*}{\begin{tabular}{@{}c@{}}#2\end{tabular}}}%
        \newcommand{\Mr}[2][3]{\mr[#1]{#2}}%
        \renewcommand{\phi}{\varphi}%
        \newcommand{\cost}{\ensuremath{\varphi+\indicator_{\overline C}}}%
        \newcommand{\club}{\(^{\clubsuit}\)}%
    %
    \begin{tabular}{@{}| c | l|c|l |@{}}
        \header{\clap{Operation}} &  \header{\((\Mon^\prime,\Com^\prime)\)\hyp{}semimonotone} & \header{\clap{Requirements}}  & \header{Reference}  \\
    \hline
    %
    % :::::::: sums ::::::::::
    %
        \(A + B\)   
        &
        \(\Mon^\prime =\Mon_A+ \Mon_B\), \(\Com^\prime = \Com_A \Box \Com_B\)
        &
        \((\Com_A,\Com_B)\in \parsumset\)    &
        \cref{prop:calculus:sum}
        \\
        \hline
        \(A \Box B\)   
        &
        \(\Mon^\prime =\Mon_A \Box \Mon_B\), \(\Com^\prime = \Com_A + \Com_B\)
        &
        \((\Mon_A,\Mon_B)\in \parsumset\)    &
        \cref{lem:calculus:parsum}
        \\
        \hline
    %
    % :::::::: composition ::::::::::
    %
        \(L^\top A L\)
        &
        \(\Mon^\prime \preceq L^\top \Mon_A L\) and \(L \Com^\prime L^\top \preceq \Com_A\)
        & - & \cref{lem:calculus:composition:1}
        \\
                    % &                                       &     &             \\
        \hline
        $L^\top \rhd A \dfn (L^\top A^{-1} L)^{-1}$
        &
        \(L \Mon^\prime L^\top \preceq \Mon_A\) and \(\Com^\prime \preceq L^\top \Com_A L\)
        & - & \cref{lem:calculus:composition:2} 
        \\%\cline{2-2}
        \hline
    %
    % :::::::: sum with linear ::::::::::
    %
        \(A + L\)
        &
        ?
        & - & ?
        \\%\cline{2-2}
        \hline
    %
    % :::::::: sum with linear ::::::::::
    %
        \(A + \alpha \I\)
        &
        \(\Mon^\prime=\MonA+\alpha(1-\epsilon\alpha)\), \(\Com^\prime = \ComA \Box \epsilon\I\)
        & \((\ComA,\epsilon\I) \in \parsumset\), \(\epsilon \in \R\) \hl{TODO: except $\nicefrac{1}{2\alpha}$ if $\alpha < 0$?}& \cref{lem:calculus:sum:identity}
        \\
        \hline\hline
    %
    % :::::::: smooth and \(\mu\)-convex ::::::::::
    %
        \(\partial f = \nabla f \)
        &
        \(\mon^\prime =  \frac{\nu_f \ell_f}{\ell_f+ \nu_f}\), \(\com^\prime = \frac{1}{\ell_f+\nu_f}\)
        & \(f\) \(\ell_f\)-smooth and \(\nu_f\)-convex, \(\nu_f\in[-\ell_f,\ell_f]\) & 
        \cref{lem:smoothhypo}
        \\%\cline{2-2}
        \hline

    %
    % :::::::: Klee ::::::::::
    %
        \(\partial(-\klee_f^{\alpha})\)
        &
        \(\mon^\prime =  0\), \(\com^\prime = -\alpha\)
        & \(f\) proper lsc cvx, \(\alpha>0\), (prox bounded  name), & 
        \cref{lem:klee:semi}
        \\%\cline{2-2}
        \hline
        \(\partial(-f)\)
        &
        \(\mon^\prime =  0\), \(\com^\prime = -\alpha\)
        &\(f\) proper lsc \(\nicefrac1{\alpha}\)-str cvx,  \(\alpha>0\) & 
        \cref{cor:strcvx:klee}
        \\%\cline{2-2}
        \hline
    \hline\hline
    \end{tabular}%
    %%<< [APPENDED to input], level=0, file=TeX/Tables/Summary.tex
    \caption[%
    Summary of calculus rules for semimonotone operators.]{%
    $L:\R^n\to \R^m$ be a linear mapping, \(A,B\) are set-valued \((\Mon_A,\Com_A)\)-semimonotone and \((\Mon_B,\Com_B)\)-semimonotone operators. 
        {\sc abbreviations:}~
        {\em cvx}: convex;~
        {\em str}: strongly;~
        {\em smooth}: Lipschitz differentiable;%
    }%
    \label{table:summary}%
\end{table}


